Multilingual and Multilabel Emotion Recognition using Virtual Adversarial Training

Virtual Adversarial Training (VAT) has been effective in learning robust models under supervised and semi-supervised settings for both computer vision and NLP tasks. However, the efficacy of VAT for multilingual and multilabel text classification has not been explored before. In this work, we explore VAT for multilabel emotion recognition with a focus on leveraging unlabelled data from different languages to improve the model performance. We perform extensive semi-supervised experiments on SemEval2018 multilabel and multilingual emotion recognition dataset and show performance gains of 6.2% (Arabic), 3.8% (Spanish) and 1.8% (English) over supervised learning with same amount of labelled data (10% of training data). We also improve the existing state-of-the-art by 7%, 4.5% and 1% (Jaccard Index) for Spanish, Arabic and English respectively and perform probing experiments for understanding the impact of different layers of the contextual models.

==> sections/extra.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|l|c|c|c|} 
\hline
\% & Method & \jindex & \microfs & \macrofs & \jindex & \microfs & \macrofs \\
 \hline
\multirow{2}{*}{10} & \supex & 44.05 & 57.86 & 40.91 & 44.05 & 57.86 & 40.91\\\cline{2-5}
&\mlvat & \textbf{46.79} & \textbf{60.36} & \textbf{44.41} & \textbf{46.79} & \textbf{60.36} & \textbf{44.41}\\
\hline
\multirow{2}{*}{25} & \supex  & 49.69 & 62.80 & 44.19 & 49.69 & 62.80 & 44.19\\\cline{2-5}
& \mlvat & \textbf{51.08} & \textbf{63.96} & \textbf{47.31} & \textbf{51.08} & \textbf{63.96} & \textbf{47.31}\\
\hline
\multirow{2}{*}{50} & \supex  & 53.95 & 66.26 & 48.57 & \supex  & 53.95 & 66.26 & 48.57\\\cline{2-5}
& \mlvat & \textbf{55.11} & \textbf{66.79} & \textbf{52.52} & \textbf{55.11} & \textbf{66.79} & \textbf{52.52}\\
\hline
\multirow{2}{*}{100} & \supex  & 55.78 & 67.41 & 50.12 & \supex  & 55.78 & 67.41 & 50.12\\\cline{2-5}
& \mlvat & \textbf{57.31} & \textbf{68.18} & \textbf{52.15} & \textbf{57.31} & \textbf{68.18} & \textbf{52.15}\\
\hline
\end{tabular}
\caption{\mlvat and Supervised (\supex) experiments on \textbf{Arabic} across different ratios of labelled examples}
\label{table:finetuned_vat_sup_ar}
\end{table}



\begin{table}[ht]

\centering
\begin{tabular}{|l|l|c|c|c|} 
 \hline
\% & Method & \jindex & \microfs & \macrofs \\
\hline
\multirow{2}{*}{10} & \supex  & 54.15 & 66.33 & 48.94\\\cline{2-5}
& \mlvat & \textbf{55.15} & \textbf{67.01} & \textbf{50.57}\\
\hline
\multirow{2}{*}{25} & \supex  & 55.11 & 66.99 & 47.83\\\cline{2-5}
& \mlvat & \textbf{56.54} & \textbf{68.52} & 51.18\\
\hline
\multirow{2}{*}{50} & \supex  & 57.20 & 69.14 & \textbf{54.14}\\\cline{2-5}
& \mlvat & \textbf{58.67} & \textbf{70.03} & \textbf{51.55}\\
\hline
\multirow{2}{*}{100} & \supex  & 59.78 & 71.19 & 53.43\\\cline{2-5}
& \mlvat& \textbf{60.70} & \textbf{71.90} & \textbf{56.10}\\
\hline
\end{tabular}
\caption{\mlvat and Supervised (\supex ) experiments on \textbf{English} across different ratios of labelled examples}
\label{table:finetuned_vat_sup_en}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{|l|l|c|c|c|} 
 \hline
\% & Method & \jindex & \microfs & \macrofs \\
 \hline
\multirow{2}{*}{10} & \supex  & 44.36 & 53.17 & 38.28\\\cline{2-5}
& \mlvat & \textbf{46.05} & \textbf{54.83} & \textbf{42.49}\\
\hline
\multirow{2}{*}{25} & \supex  & \textbf{52.89} & \textbf{61.30} & 48.99\\\cline{2-5}
& \mlvat & 52.05 & 60.17 & \textbf{49.15}\\
\hline
\multirow{2}{*}{50} & \supex  & 55.17 & 63.20 & 51.70\\\cline{2-5}
& \mlvat  & \textbf{55.70} & \textbf{63.39} & \textbf{54.19}\\
\hline
\multirow{2}{*}{100} & \supex  & \textbf{57.04} & \textbf{65.31} & 51.53\\\cline{2-5}
& \mlvat  & 56.89 & 64.89 & \textbf{51.77}\\
\hline
\end{tabular}
\caption{\mlvat and Supervised (\supex) experiments on \textbf{Spanish} across different ratios of labelled examples}
\label{table:finetuned_vat_sup_es}
\end{table}




==> sections/extras-poster.tex <==




\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|c|} 
 \hline
Model & JI & MiF1 & MaF1 \\
\hline
mlVAT & \textbf{60.7} & \textbf{71.9} & \textbf{56.1}\\
\hline
XLM-Tw & 59.8 & 71.2 & 53.4\\
\hline
E-BERT & 59.1 & 70.4 & 53.3\\
\hline
\end{tabular}
\caption{Results on English}
\label{table:finetuned_results_en}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|c|} 
 \hline
Model & JI & MiF1 & MaF1 \\
\hline
mlVAT & 56.9 & 64.9 & \textbf{51.8} \\
\hline
XLM-Tw & \textbf{57.0} & \textbf{65.3} & 51.5\\
\hline
BetoBERT & 52.7 & 60.8 & 48.7\\
\hline
\end{tabular}
\caption{Results on Spanish}
\label{table:finetuned_results_es}
\end{table}


\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|c|} 
 \hline
Model & JIx & MiF1 & MaF1 \\
\hline
mlVAT & \textbf{57.3} & \textbf{68.2} & \textbf{52.2}\\
\hline
XLM-Tw & 55.8 & 67.4 & 50.1\\
 \hline
AraBERT & 54.3 & 65.9 & 49.0\\
\hline
\end{tabular}
\caption{Results on Arabic}
\label{table:finetuned_results_ar}
\end{table}


\begin{table}[ht]
\centering
\begin{tabular}{|l|l|c|c|c|} 
\hline
\% & Method & JI & MiF1 & MaF1 \\
 \hline
\multirow{2}{*}{10} & Sup & 44.1 & 57.9 & 40.9\\
&mlVAT & \textbf{46.8} & \textbf{60.4} & \textbf{44.4}\\
\hline
\multirow{2}{*}{25} & Sup  & 49.7 & 62.8 & 44.2\\
& mlVAT & \textbf{51.1} & \textbf{64.0} & \textbf{47.3}\\
\hline
\multirow{2}{*}{50} & Sup  & 54.0 & 66.3 & 48.6\\
& mlVAT & \textbf{55.1} & \textbf{66.8} & \textbf{52.5}\\
\hline
\multirow{2}{*}{100} & Sup  & 55.8 & 67.4 & 50.1\\
& mlVAT & \textbf{57.3} & \textbf{68.2} & \textbf{52.2}\\
\hline
\end{tabular}
\caption{\mlvat and Supervised (\supex) experiments on \textbf{Arabic} across different ratios of labelled examples}
\label{table:finetuned_vat_sup_ar}
\end{table}


\begin{table*}[h]
\centering
\begin{tabular}{|l|l|c|c|c||c|c|c|} 
\hline
 \multirow{2}{*}{\%} & \multirow{2}{*}{Method} & \multicolumn{3}{c||}{English} & \multicolumn{3}{c|}{Spanish} \\\cline{3-8}
 &  & JI & MiF1 & MaF1 & JI & MiF1 & MaF1 \\
 \hline
\multirow{2}{*}{10} & Sup & 54.2 & 66.3 & 48.9 & 44.4 & 53.2 & 38.3\\
&mlVAT & \textbf{55.2} & \textbf{67.0} & \textbf{50.6} & \textbf{46.1} & \textbf{54.8} & \textbf{42.5}\\
\hline
\multirow{2}{*}{25} & Sup  & 55.1 & 66.9 & 47.8 & \textbf{52.9} & \textbf{61.3} & 48.9\\
& mlVAT & \textbf{56.5} & \textbf{68.5} & \textbf{51.2} & 52.1 & 60.2 & \textbf{49.2}\\
\hline
\multirow{2}{*}{50} & Sup  & 57.2 & 69.1 & \textbf{54.1} & 55.2 & 63.2 & 51.7\\
& mlVAT & \textbf{58.7} & \textbf{70.0} & 51.6 & \textbf{55.7} & \textbf{63.4} & \textbf{54.2}\\
\hline
\multirow{2}{*}{100} & Sup & 59.8 & 71.2 & 53.4 & \textbf{57.0} & \textbf{65.3} & 51.5\\
& mlVAT & \textbf{60.7} & \textbf{71.9} & \textbf{56.1} & 56.9 & 64.9 & \textbf{51.8}\\
\hline
\end{tabular}
\caption{\mlvat and Supervised (\supex) experiments on \textbf{Arabic} across different ratios of labelled examples}
\label{table:finetuned_vat_sup_ar}
\end{table*}


